Ref-GS: Directional Factorization for 2D Gaussian Splatting

In this paper, we introduce Ref-GS, a novel approach for directional light factorization in 2D Gaussian splatting, which enables photorealistic view-dependent appearance rendering and precise geometry recovery. Ref-GS builds upon the deferred rendering of Gaussian splatting and applies directional encoding to the deferred-rendered surface, effectively reducing the ambiguity between orientation and viewing angle. Next, we introduce a spherical Mip-grid to capture varying levels of surface roughness, enabling roughness-aware Gaussian shading. Additionally, we propose a simple yet efficient geometry-lighting factorization that connects geometry and lighting via the vector outer product, significantly reducing renderer overhead when integrating volumetric attributes. Our method achieves superior photorealistic rendering for a range of open-world scenes while also accurately recovering geometry.

==> sec/3_Method.tex <==
\section{Method}
\label{sec:method}


\subsection{Preliminaries}
\noindent\textbf{2D Gaussian Splatting.} Our reconstruction stage builds upon the state-of-the-art point-based renderer with the splendid geometry performance, 2DGS~\cite{huang20242d}. 2DGS is defined by several key components: the central point $\mathbf{p}_k$, two principal tangential vectors $\mathbf{t}_u$ and $\mathbf{t}_v$ that determine its orientation, and a scaling vector $\mathbf{S} = (s_u, s_v)$ controlling the variances of the 2D Gaussian distribution. 

2D Gaussian Splatting represents the scene's geometry as a set of 2D Gaussians. A 2D Gaussian is defined in a local tangent plane in world space, parameterized as follows:
\begin{align}
P(u,v) &= \mathbf{p}_k + s_u \mathbf{t}_u u + s_v \mathbf{t}_v v .
\label{eq:plane-to-world}
\end{align}
For the point $\mathbf{u}=(u,v)$ in $uv$ space, its 2D Gaussian value can then be evaluated using the standard Gaussian function:
\begin{equation}
\mathcal{G}(\mathbf{u}) = \exp\left(-\frac{u^2+v^2}{2}\right).
\label{eq:gaussian-2d}
\end{equation}
The center $\mathbf{p}_k$, scaling $(s_u, s_v)$, and the rotation $(\mathbf{t}_u, \mathbf{t}_v)$ are learnable parameters. 
Each 2D Gaussian primitive has opacity $\alpha$ and view-dependent appearance $\mathbf{c}$ with spherical harmonics. 
For volume rendering, Gaussians are sorted according to their depth value and composed into an image with front-to-back alpha blending:
\begin{equation}
\label{2dgs}
\mathbf{c}(\mathbf{x}) = \sum_{i=1} \mathbf{c}_i \alpha_i \mathcal{G}_i(\mathbf{u}(\mathbf{x})) \prod_{j=1}^{i-1} (1 - \alpha_j \mathcal{G}_j(\mathbf{u}(\mathbf{x}))).
\end{equation}
where $\mathbf{x}$ represents a homogeneous ray emitted from the camera and passing through $uv$ space.

\noindent\textbf{View-dependent Appearance.} Ref-NeRF decomposes the color $\mathbf{c}(\mathbf{x}, \omega_i)$ (dependent on the viewing direction $\omega_i$) into a diffuse color $\mathbf{c}_d$, specular tint $\mathbf{k}_s$, and specular color $\mathbf{c}_s$ queried in reflected direction $\omega_r \in \mathbb{R}^3$ with surface normal $\mathbf{n} \in \mathbb{R}^3$:
%
\begin{equation}
\begin{aligned}
\mathbf{c}(\mathbf{x}, \omega_i) &= \mathbf{c}_d(\mathbf{x}) + \mathbf{k}_s(\mathbf{x})\mathbf{c}_s(\mathbf{x}, \omega_r) \\
\omega_r &= \omega_i-2(\omega_i\cdot\mathbf{n})\mathbf{n}
\end{aligned}
\end{equation}
%
Inspired by the deferred shading techniques from the gaming industry, we adopt a similar approach to structure outgoing radiance in the image space. Here, the diffuse image $\mathbf{I}_d$ is obtained directly through gaussian splatting; the specular color is decoded from the shader $f_\theta$ that conditions on spatial feature $\mathbf{K} \in \mathbb{R}^{H \times W \times N}$, directional feature $\mathbf{S} \in \mathbb{R}^{H \times W \times C}$:
%
\begin{equation}
\label{deferredShading}
\mathbf{I} = \mathbf{I}_d + f_\theta(\mathbf{S}, \mathbf{K} \circ \mathbf{S})
\end{equation}
%
where $\circ$ refers to the outer product, This low-rank tensor factorization can compensate for the unrealistic rendering caused by the assumption that \textit{alllights in the scene come from infinity}, especially when light sources or other objects are in close proximity to the target object.


\subsection{Feature Deferred Shading}
To recover the view-dependent appearance, we incorporate a rendering model with the deferred shading technique. We first render a G-buffer containing per-pixel features, normals,and materials. Then, the G-buffer is processed by a learned shader $f_\theta$. Specifically, features map $\mathbf{K}$ is obtained through feature splatting, similar to gaussian splatting, except that the RGB color $\mathbf{c}_i$ in Eq.\ref{2dgs} is now replaced by features $\mathbf{k}_{i} \in \mathbb{R}^N$. Moreover, we treat the normal $n_{i}$ and roughness $\rho_{i}$ as an attribute of each Gaussian and use gaussian splatting to render the normal map $\mathbf{N}$ and roughness map $\mathbf{M}$. directional feature $\mathbf{S}$ is query from $\operatorname{Sph-Mip}$ encoding.

Finally, the reflection direction is calculated based on the normals and the view direction. Given the surface roughness $\rho$, we then query directional features $\mathbf{S}$ from $\operatorname{Sph-Mip}$ encoding.

% Neural deferred shading (NDS) optimizes an explicit mesh that is rasterized to generate a geometry buffer (G-buffer) that contains per-pixel positions, normals, and mask information. Then, the G-buffer is processed by a learned shader.

% it takes G-buffer as input and obtains final image $\mathbf{I}$ through a learned shader. Our key insight is to recover the geometry, materials and features from the G-buffer and

% Inspired by the deferred shading techniques from the gaming industry, we propose a G-buffer based view-dependent appearance.


% Different from neural deferred shading, it takes geometry buffer (G-buffer) as input and obtains final image $\mathbf{I}$ through a learned shader. Our input to the shader $f_\theta$ is a feature map encode information related to view direction and geometry, in Eq.\ref{deferredShading}. $\mathbf{K}$ is obtained through feature splatting, similar to gaussian splatting, except that the RGB color $\mathbf{c}_i$ in Eq.\ref{2dgs} is now replaced by features $\mathbf{k}_{i} \in \mathbb{R}^N$.

% We represent the shader $f_\theta$ as a tiny MLP, with $\theta$ as the parameters of the fully-connected layers. At the same time, since the MLP network $f_\theta$ is shallow and narrow, our method still achieves fast rendering speed.

% \subsection{Feature Deferred Rendering}
% Different from neural deferred shading, it takes geometry buffer (g-buffer) as input and obtains final image $\mathbf{I}$ through a learned shader. Our input to the shader $f_\theta$ is a feature map $\mathbf{F}$ encode information related to view direction and geometry. Specifically, the feature map $\mathbf{F}$ consist of three parts:
% %
% \begin{equation}
% \mathbf{F} = [\mathbf{F}^{ref}, \mathbf{F}^{\circ}]
% \end{equation}

% % where $\mathbf{F}^{base} \in \mathbb{R}^4$ is obtained through feature splatting, similar to gaussian splatting, except that the RGB color $\mathbf{c}_i$ in Eq.\ref{2dgs} is now replaced by features $\mathbf{f}_{i}^{base}$.
% %
% \begin{equation}
% \mathbf{I} = f_\theta(\mathbf{F})
% \end{equation}
% %
% We represent the shader $f_\theta$ as a tiny MLP, with $\theta$ as the parameters of the fully-connected layers. At the same time, since the MLP network $f_\theta$ is shallow and narrow, our method still achieves fast rendering speed.

\subsection{Spherical-Mip Encoding}

Given the G-buffer, the normals $\mathbf{n}=\mathbf{N}(u, v)$ and roughness $\rho=\mathbf{M}(u, v)$ are obtained by indexing the corresponding pixel values at the coordinate $(u, v)$, then we can also obtain the reflection direction $\omega_r$.

Brute-force integrals over the environment map are expensive, hence we propose a novel $\operatorname{Sph-Mip}$ encoding parameterized by \textit{Lat.-Long.} trainable mipmap $\mathcal{M}$ that is trained to directly output the integrated illumination feature vectors $\mathbf{s}$ conditioned on the surface roughness $\rho$ evenly spaced in $[0,1]$ and reflective direction $\omega_r$ :
%
\begin{equation}
\mathbf{s} = \operatorname{Sph-Mip}(\omega_r, \rho, \mathcal{M})
\end{equation}
%
For global mipmap, the base level $\mathcal{M}^{L_0}$ is a feature map with the shape of $H_\mathcal{M} \times W_\mathcal{M} \times C$, where $H_\mathcal{M}, W_\mathcal{M}, C$ are the height, width, and number of channels, respectively.
%
The base level $\mathcal{M}^{L_0}$ can be trained during the reconstruction, and other levels ($\mathcal{M}^{L_i}, i={1,2,...,N}$) are derived from the previous level $\mathcal{M}^{L_{i-1}}$ by downscaling $2\times$ along the height and width.

To query the feature vectors $\mathbf{s}$ corresponding to the  Cartesian coordinates $\omega_r$, we first calculate its corresponding spherical coordinates $(\theta, \phi)$ using the following equations:
\begin{equation}
    \begin{aligned}
    \theta &= \text{arccos} \left(\frac{\omega_r^z}{\sqrt{{\omega_r^x}^2+{\omega_r^y}^2+{\omega_r^z}^2}}\right)  \in \left [0, \pi \right ], \\
    \phi &= \text{arctan2} \left(\frac{{\omega_r^y}}{{\omega_r^x}}\right)  \in \left [-\pi, \pi \right ],    
    \end{aligned}
\end{equation}
Given the surface roughness $\rho$, we find the two nearest levels of the mipmap $\mathcal{M}^{\lfloor \rho \rfloor}$ and $\mathcal{M}^{\lceil \rho \rceil}$; and then we project the center coordinate $(\theta, \phi)$ to the two levels of the mipmap; finally, we can get the feature vector $\mathbf{f}$ from the mipmap by the trilinear interpolation.

\section{}
